Crafting Generative Art through Genetic Improvement: Managing Creative Outputs in Diverse Fitness Landscapes

Generative art is a rules-driven approach to creating artistic outputs in various mediums. For example, a fluid simulation can govern the flow of colored pixels across a digital display or a rectangle placement algorithm can yield a Mondrian-style painting. Previously, we investigated how genetic improvement, a sub-field of genetic programming, can automatically create and optimize generative art drawing programs. One challenge of applying genetic improvement to generative art is defining fitness functions and their interaction in a many-objective evolutionary algorithm such as Lexicase selection. Here, we assess the impact of each fitness function in terms of the their individual effects on generated images, characteristics of generated programs, and impact of bloat on this specific domain. Furthermore, we have added an additional fitness function that uses a classifier for mimicking a human's assessment as to whether an output is considered as "art." This classifier is trained on a dataset of input images resembling the glitch art aesthetic that we aim to create. Our experimental results show that with few fitness functions, individual generative techniques sweep across populations. Moreover, we found that compositions tended to be driven by one technique with our current fitness functions. Lastly, we show that our classifier is best suited for filtering out noisy images, ideally leading towards more outputs relevant to user preference.

==> sections/4-bloat.tex <==
In prior experiments we did not factor in the amount of bloat that occurred within generated outputs as we assumed that the inclusion of more techniques would lead to more interesting outputs.
However, such an approach does not lend itself well to artistic styles other than glitch art and as such necessitates an investigation into superfluous outputs.
We next discuss the average number of function calls per experimental configuration and discuss approaches for culling bloat.

% \begin{table}[htb!]
% % \centering
% \begin{tabular}{|| c | c ||| c | c ||| c | c ||| c | c ||} 
%  \hline
%  ID & $avg_{ti}$ & ID & $avg_{ti}$ & ID & $avg_{ti}$ & ID & $avg_{ti}$ \\ \hline \hline
%  $EC_{1}$ & X & $EC_{17}$ & X & $EC_{33}$ & X & $EC_{49}$ & X \\ \hline
%  $EC_{2}$ & X & $EC_{18}$ & X & $EC_{34}$ & X & $EC_{50}$ & X \\ \hline
%  $EC_{3}$ & X & $EC_{19}$ & X & $EC_{35}$ & X & $EC_{51}$ & X \\ \hline
%  $EC_{4}$ & X & $EC_{20}$ & X & $EC_{36}$ & X & $EC_{52}$ & X \\ \hline
%  $EC_{5}$ & X & $EC_{21}$ & X & $EC_{37}$ & X & $EC_{53}$ & X \\ \hline
%  $EC_{6}$ & X & $EC_{22}$ & X & $EC_{38}$ & X & $EC_{54}$ & X \\ \hline
%  $EC_{7}$ & X & $EC_{23}$ & X & $EC_{39}$ & X & $EC_{55}$ & X \\ \hline
%  $EC_{8}$ & X & $EC_{24}$ & X & $EC_{40}$ & X & $EC_{56}$ & X \\ \hline
%  $EC_{9}$ & X & $EC_{25}$ & X & $EC_{41}$ & X & $EC_{57}$ & X \\ \hline
%  $EC_{10}$ & X & $EC_{26}$ & X & $EC_{42}$ & X & $EC_{58}$ & X \\ \hline
%  $EC_{11}$ & X & $EC_{27}$ & X & $EC_{43}$ & X & $EC_{59}$ & X \\ \hline
%  $EC_{12}$ & X & $EC_{28}$ & X & $EC_{44}$ & X & $EC_{60}$ & X \\ \hline
%  $EC_{13}$ & X & $EC_{29}$ & X & $EC_{45}$ & X & $EC_{61}$ & X \\ \hline
%  $EC_{14}$ & X & $EC_{30}$ & X & $EC_{46}$ & X & $EC_{62}$ & X \\ \hline
%  $EC_{15}$ & X & $EC_{31}$ & X & $EC_{47}$ & X & $EC_{63}$ & X \\ \hline
%  $EC_{16}$ & X & $EC_{32}$ & X & $EC_{48}$ & X & $EC_{64}$ & X \\ \hline
% \end{tabular}
% \caption{Average number of technique invocations ($avg_{ti}$) per experimental configuration (c.f., ~\ref{table:expr-conf}).}
% \label{table:ffs}
% \end{table}

As can be seen, ...\todo{scan generated code for length}

Typically, bloat has a negative impact on solutions in that unnecessary and/or invalid code may be executed, leading to significant issues (in terms of behavior or performance) on the system under execution.
However, for the purposes of creating generative art bloat typically manifests in terms of overly-busy or cluttered outputs (some of which are aesthetically-interesting in and of themselves).
Even so, our goal is to reduce bloat as much as possible.

% Former ways of handling this...\todo{lookup bloat related work}
Program bloat is a well-studied topic within the genetic programming domain.

\texttt{GenerativeGI} uses GE as a mechanism for evolution and therefore can use constraints within the input grammar definition to further reduce unnecessary calls.
Presently, all techniques are considered to be top-level functions and each have an equal chance of being incorporated within the generated program.
However, some functions that apply filters (e.g., OpenCV's watercolor filter~\cite{opencv_library}) do not necessarily impact the visuals on a blank canvas and work best when prior functions have been called.
An optimal grammar definition can therefore be used to minimize ``obvious'' bloat issues while still retaining the power of the evolutionary process.

Another mechanism for bloat reduction can be to scan generated programs for redundant or conflicting calls.
At present, there are no interactions between drawing techniques (e.g., a particle from a flow field will not recognize that a circle has been drawn and avoid it) and as such overlapping techniques further contribute to noise.
Unless if otherwise desirable by the designer, a post-processing pass on the generated program to remove duplicates can be helpful in reducing unnecessary noise.\todo{Is this a good thing to check for art v not art?}
For example, drawing two flow fields within the same program can cause significant overlap and negate the effects of each.

% Ways to fix it:
% lookup related works here
% - incorporate bloat metrics as fitness functions
% - scan for redundant calls
% - upgrade grammar to forcibly reduce bloat


% bloat papers
% Avoiding the Bloat with Stochastic Grammar-based Genetic Programming
\cite{ratle2001avoiding}
% Operator equalisation for bloat free genetic programming and a survey of bloat control methods
\cite{silva2012operator}
% A Simple but Theoretically-motivated Method to Control Bloat in Genetic Programming
\cite{poli2003simple}
% Dynamic limits for bloat control in genetic programming and a review of past and current bloat theories
\cite{silva2009dynamic}
% Quadratic Bloat in Genetic Programming
\cite{langdon2000quadratic}
% A Comparison of Bloat Control Methods for Genetic Programming
\cite{luke.2006}


==> sections/5-related.tex <==
% This section discusses related work in terms of artificial intelligence and other search-based artistic techniques.

% \subsubsection{Artificial Intelligence}

% \subsubsection{Search-Based Artistic Techniques}

% \todo{Could move to BG if space is a concern}

==> sections/timings.tex <==
50 invocations with different seeds

stippled: Average [0.035771937370300294] Minimum [0.03402566909790039] Maximum [0.039324283599853516]
wolfram-ca: Average [0.009601960182189942] Minimum [0.008081197738647461] Maximum [0.012642860412597656]
flow-field: Average [10.019215846061707] Minimum [9.630614042282104] Maximum [10.79770040512085]
pixel-sort: Average [0.35263049602508545] Minimum [0.16085195541381836] Maximum [0.6415228843688965]
drunkardsWalk: Average [0.4087705326080322] Minimum [0.025861263275146484] Maximum [1.2039620876312256]
dither: Average [0.14172054290771485] Minimum [0.00671696662902832] Maximum [0.25691676139831543]
flow-field-2: Average [0.8063605642318725] Minimum [0.26746439933776855] Maximum [1.8754549026489258]
circle-packing: Average [0.09543720245361328] Minimum [0.04361295700073242] Maximum [0.1746501922607422]
rgb-shift: Average [0.10608686447143555] Minimum [0.10031890869140625] Maximum [0.11845684051513672]
noise-map: Average [2.876542816162109] Minimum [2.790560007095337] Maximum [3.076564073562622]
oil-painting-filter: Average [0.019672136306762695] Minimum [0.012178421020507812] Maximum [0.028307676315307617]
watercolor-filter: Average [0.07334259033203125] Minimum [0.06477165222167969] Maximum [0.08446645736694336]
pencil-filter: Average [0.031008539199829103] Minimum [0.025830507278442383] Maximum [0.037772417068481445]
walkers: Average [0.10780280113220214] Minimum [0.025573253631591797] Maximum [0.20152997970581055]
basic_trig: Average [0.04961829662322998] Minimum [0.010504484176635742] Maximum [0.08861875534057617]

-------

100 invocations with different seeds
stippled: Average [0.03324298620223999] Minimum [0.029510974884033203] Maximum [0.04350137710571289]
wolfram-ca: Average [0.008807711601257324] Minimum [0.006944894790649414] Maximum [0.014931201934814453]
flow-field: Average [11.461736407279968] Minimum [10.799420595169067] Maximum [12.309314012527466]
pixel-sort: Average [0.27940509796142576] Minimum [0.1367168426513672] Maximum [0.5655436515808105]
drunkardsWalk: Average [0.15341667890548705] Minimum [0.011942386627197266] Maximum [0.4486846923828125]
dither: Average [0.10065114736557007] Minimum [0.005785226821899414] Maximum [0.18413209915161133]
flow-field-2: Average [0.7667304134368896] Minimum [0.3077201843261719] Maximum [1.8734347820281982]
circle-packing: Average [0.13939666032791137] Minimum [0.051950931549072266] Maximum [0.2627599239349365]
rgb-shift: Average [0.11628097772598267] Minimum [0.10777878761291504] Maximum [0.19592618942260742]
noise-map: Average [2.855066478252411] Minimum [2.768089532852173] Maximum [3.1340460777282715]
oil-painting-filter: Average [0.02170093297958374] Minimum [0.011111021041870117] Maximum [0.039720773696899414]
watercolor-filter: Average [0.12032846689224243] Minimum [0.09889817237854004] Maximum [0.6368343830108643]
pencil-filter: Average [0.05565020799636841] Minimum [0.03674459457397461] Maximum [0.5685403347015381]
walkers: Average [0.04016606569290161] Minimum [0.01261758804321289] Maximum [0.07744574546813965]
basic_trig: Average [0.038989150524139406] Minimum [0.008720636367797852] Maximum [0.07140445709228516]
